Derived Equivalent Calabi-Yau 3-folds from Cubic 4-folds

We describe pretty examples of derived equivalences and autoequivalences of Calabi-Yau threefolds arising from pencils of cubic fourfolds. The cubic fourfolds are chosen to be special, so they have an associated K3 surface. Thus a pencil gives rise to two different Calabi-Yau threefolds: the associated pencil of K3 surfaces, and the baselocus of the original pencil - the intersection of two cubic fourfolds. They both have crepant resolutions which are derived equivalent.

==> computation.tex <==
Recall we blow up a point in $\P^5$ and project away $\rho\colon P \to \P^4$.
We then blow up $X$ obtaining $\H \subset P \times \P^1$.
So we have the following maps.
\[
    \begin{tikzcd}
    D \ar{r}{i} & 
    \H \ar{r}{\alpha} \ar[bend right]{rr}{\gamma} &
    P \times \P^1 \ar{r}{\rho} &
    \P^4 \times \P^1
    \end{tikzcd}
\]
where $\rho$ should really be $\rho\times \id$ and $D$ fits in a fibre square
\[
\begin{tikzcd}
D \ar{d}[swap]{\delta} \ar{r}{i} & \H \ar{d}{\gamma} \\
Y \ar{r}{j} & \P^4\times \P^1
\end{tikzcd}
\]
where we see $\H = \Bl_Y \P^4 \times \P^1$, with exceptional locus $D$.

\bigskip
We are now trying to compute the rank of whatever happens to $\O_x$ for a random point $x \in X$.
After pulling up, pushing in $\H$ and mutating, we end up with some element of the K-group $\E$, which consists of a bunch of line bundles plus things like $\O_F$, where $F$ is the $\P^1$ fibre over $x$.

Now, projecting to $Y$ means first doing $i^!$, which is just tensoring with some line bundles and shifting by minus one.


If $\E$ is a rank $r+1$ vector bundle on some variety $X$, with projectivization $\pi \colon \P(\E) \to X$ then

\[ \pi_* \O_\pi(d) = \Sym^d \E^\vee \oplus \bigg( \det \E \otimes  \Sym^{-d -r -1} \E [-r] \bigg). \]


Then, since $\rho$ is the bundle $\P( \O(1,0) \oplus \O)$
\[ \rho_*\O_\rho(z) =
\bigoplus_{0 \leq h \leq z} \O(-h,0) \oplus
\bigoplus_{0 \leq k \leq -z -2} \O(1+k,0)[-1]
\]

Keeping notation from the paper, by $\O(x,y)(ze)$ we mean the bundle on $\H$ given by pulling $\O(x)$ up from $\P^5$, $\O(ze)$ from $P$ and $\O(y)$ from $\P^1$.
When we write $\rho^*\O(x,y)$ or $\gamma^*\O(x,y)$ then $\O(x,y)$ is the usual line bundle on $\P^4 \times \P^1$.
\begin{align*}
    \O(e) &= \O_\rho(1) \\
    \O(x,y)(ze) &= \gamma^* \O(x,y)\otimes \alpha^* \O_\rho(x+z) \\
    \O(-\H) &= \O(-3,-1)(2e)\\
    K_\H &= \O(-3,-1)(2e) \\
        &= \O(-5,-2)(5e)(D) \\
        \O(-D) &= 
            \O(-2,-1)(3e) \\
        K_D &= i^* \O(-1,0)(-e) \\
        i^!(-) &= \otimes K_D [4] \circ i^* \circ \otimes K_\H^{-1} [-5] \\
        &= i^*\big( (-) \otimes \O(2,1)(-3e) \big)[-1]
\end{align*}

\subsection*{Mutations}
The starting point is this sod.
\begin{multline*}
\Langle\O,\O(1,0),\O(2,0),\O_e,\O_e(-e), \\
D(X),\O(0,1),\O(1,1),\O(2,1),\O_e(0,1),\O_e(-e)(0,1)\Rangle.
\end{multline*}
We mutate $D(X)$ to the right and perform other operations which do not affect $D(X)$.
Then we left mutate four times to obtain this other sod.
\begin{multline*}
\Langle\O,\O(1,0)(-e),\O(2,0)(-2e),\O(0,1),\O(1,1)(-e), \\
\O(2,1)(-2e),D(X),\O(1,0),\O(2,0)(-e),\O(1,1),\O(2,1)(-e)\Rangle.
\end{multline*}
After this, we project down to $D(Y)$.

All computations will be done in the K-group, so that
\begin{align*}
L_E F = F - \Hom(E,F) \cdot E \\ 
R_E F = F - \Hom(F,E) \cdot E
\end{align*}
Projection down to $D(Y)$ is given by $\delta_* i^!$.
In the end we want to compute the resulting Euler characteristic, which is done by pushing down to a point.
Hence, we might as well first push into $\P^4\times \P^1$ using $j_*$, so at the end of the day we want to compute $H^*(\P^4\times \P^1, \gamma_* i_* i^!)$ which is the same as doing
\begin{align}\label{thisthing}
H^*(\H,-) - H^*(\H, (-) \otimes \O(2,1)(-3e)).
\end{align}


\subsection*{First mutations}
We start with the skyscraper of some point $p \in X$ and pull it up to $\H$.
This is $\O_F$, the structure sheaf a copy of a fibre $F = \{p\} \times L$.
We note that
\[ \O_F \otimes \O(x,y)(ze) = \O_F(y) \]
where by the RHS we mean $\O_L(y)$ pushed forward to the fibre $F$.

For the first sod, instead of mutating right we mutate left and then tensor with the anticanonical.
We need to perform the following left mutations on $\O_F$:
\begin{itemize}
\item $\O_e(-e)$
\item $\O_e$
\item $\O(2,0)$
\item $\O(1,0)$
\item $\O$
\end{itemize}
Call these mutations $\nu_1,\ldots,\nu_5$.
\bigskip

$\Hom(\O_e(-e), \O_F) = 0$
\begin{flalign}
&& \nu_1 \O_F = \O_F
\end{flalign}
$\Hom(\O_e,\O_F) =0$
\begin{flalign}
&& \nu_2\nu_1 \O_F = \O_F
\end{flalign}
$\Hom(\O(2,0),\O_F)= 1$,
\begin{flalign}
&&\nu_3\nu_2\nu_1 \O_F = \O_F - \O(2,0)
\end{flalign}

$\Hom(\O(1,0),\O_F)=1$
    
$\Hom(\O(1,0),\O(2,0))=6$

\begin{flalign}
&&\nu_4\nu_3\nu_2\nu_1 \O_F = \O_F + 5\O(1,0) - \O(2,0)
\end{flalign}

$\Hom(\O,\O_F) = 1$

$\Hom(\O,\O(1,0))=6$

$\Hom(\O,\O(2,0))= 21$

\begin{flalign}
&&\nu_5\nu_4\nu_3\nu_2\nu_1 \O_F = \O_F +5 \O(1,0) - 10\O - \O(2,0)
\end{flalign}

\subsection*{Some code}
I used magma to do the arithmetic.
The full script can be found at the end of this pdf.
The first line of the code computes dimensions of symmetric powers in terms of binomials, the second and third compute cohomology of line bundles on $\P^4$ and $\P^1$.
Then we have a bit which computes $H^*(P\times \P^1, \rho^*\O(x,y)\otimes \O_\rho(z)$.

\begin{verbatim}
cohPP1 := function(v)
    if v[3] eq -1 then return 0;
    elif v[3] ge 0 then
        tmp1 := &+[cohP4(v[1]-h) : h in [0..v[3]]];
        return cohP1(v[2])*tmp1;
    elif -v[3] -2 ge 0 then
        tmp2 := &+[cohP4(v[1]+k+1) : k in [0..-v[3]-2]];
		return -cohP1(v[2])*tmp2;
    end if;
end function;
\end{verbatim}
What's it saying is that it takes as input $v$, which has three components $v[1],v[2],v[3]$ (corresponding to $x,y,z$) and spits out a number using the formula
\begin{align*}
H^*(\P^1,\O(y)) \cdot
\left[ 
    \sum_{0 \leq h \leq z} H^*(\P^4,\O(x-h)
    \quad-\sum_{0 \leq k \leq -z-2} H^*(\P^4,\O(x+k+1)
\right].
\end{align*}

\bigskip
Then we have 
\begin{verbatim}
cohH := function(v)
    u := [v[1],v[2],v[1]+v[3]];
    w := [v[1]-3,v[2]-1,v[1]+v[3]-1];
    return cohPP1(u) - cohPP1(w);
end function;
\end{verbatim}
which is saying
\[ H^*(\H,\O(x,y)(ze)) = H^*(P\times \P^1, \rho^*\O(x,y)\otimes \O_\rho(x+z)) - H^*(P\times \P^1, \rho^* \O(x-3,y-1) \otimes \O_\rho(x+z-1) \]
using that $\O(x,y)(ze) = \gamma^*\O(x,y)\otimes \alpha^* \O_\rho(x+z)$ and $\O_\H = \O - \O(-3,-1)(2e)$ in the K-group.

Finally we have the bits which compute the hom spaces.
\begin{verbatim}
hom := function(v,w)
    return cohH(w-v);
end function;

homF := func<v,x | cohP1(x-v[2]) >;
\end{verbatim}
where the last function knows that the second variable is not some $\O(x,y)(ze)$ but rather $\O_F(x)$.




\subsection*{Second mutations part 1}
First we tensor with the anticanonical, obtaining
\begin{flalign}
&& \xi\coloneqq \O_F(1) + 5\O(4,1)(-2e) -10 \O(3,1)(-2e) - \O(5,1)(-2e)
\end{flalign}
and then left mutate past 
\begin{itemize}
\item $\O(2,1)(-e)$
\item $\O(1,1)$
\item $\O(2,0)(-e)$
\item $\O(1,0)$
\end{itemize}

So we have eight sheaves $A_i$ in the K-group, counted with multiplicities $a_i$.
For example, $[4,1,-2]$ corresponds to $\O(4,1)(-2e)$, which appears with multiplicity $5$.
The first vector plays a special role because it's $\O_F(1)$, but the code which follows knows that.
\begin{verbatim}
a1 := 1;
A1 := 1;

a2 := 5;
A2 := Vector([4,1,-2]);

a3 := -10;
A3 := Vector([3,1,-2]);

a4 := -1;
A4 := Vector([5,1,-2]);

a5 := 0;
A5 := Vector([2,1,-1]);

a6 := 0;
A6 := Vector([1,1,0]);

a7 := 0;
A7 := Vector([2,0,-1]);

a8 := 0;
A8 := Vector([1,0,0]);

A := [Vector([0,0,0]),A2,A3,A4,A5,A6,A7,A8];
a := [a1,a2,a3,a4,a5,a6,a7,a8];
\end{verbatim}
To perform the first mutation, we need to know what the multiplicity $a_5$ should be, so we compute by adding the dimension of the relevant hom spaces together.
\begin{verbatim}
a5 := -(homF(A5,A1) + &+[a[i]*hom(A5,A[i]) : i in [2..4]]);
a := [a1,a2,a3,a4,a5,a6,a7,a8];
\end{verbatim}
where the last line is to tell magma that $a_5$ has been updated (it's no longer zero).
We repeat the same for the other three mutations.

Finally, we want to project down to $Y$ and compute the Euler characteristic.
And, using \eqref{thisthing}, we can use the function
\begin{verbatim}
Gamma := func< v | cohH(v) - cohH(v+Vector([2,1,-3])) >;
\end{verbatim}

So, the number we are after is given by
\begin{verbatim}
r1 := a1*(cohP1(A1) - cohP1(A1+1)) + &+[a[i]*Gamma(A[i]) : i in [2..8]];

print "Left mutating we get", r1;
\end{verbatim}

\subsection*{Second mutations part 2}
To crosscheck this, as you suggested, we compute the same thing by right mutating six times (instead of tensoring and left mutating four times).
So, we start with
\[ \O_F +5 \O(1,0) - 10\O - \O(2,0)\]
and then right mutate past
\begin{itemize}
\item $\O$
\item $\O(1,0)(-e)$
\item $\O(2,0)(-2e)$
\item $\O(0,1)$
\item $\O(1,1)(-e)$
\item $\O(2,1)(-2e)$
\end{itemize}

The code is essentially the same, the only thing is that homs now go in the opposite direction.
We also need
\[\Hom(\O_F(x),\O(a,b)(ce)) = H^*(\P^1,b-x-1).\]
which, if $\beta\colon \O_{\P^1} \to \H$ is the inclusion of the fibre $F$, follows from $\Hom(\O_F, E) = H^*(\P^1, \beta^! E)$ plus the formula $\beta^! = \D_{\P^1} \beta^! \D_\H^{-1}$, which we also used for the inclusion $i\colon D \to \H$ (so if I got this wrong, the I got the other wrong as well).
This is written up as 
\begin{verbatim}
Fhom := func< x,v | cohP1(v[2]-x-1) >;
\end{verbatim}


\subsection*{Conclusion}
What I did is run the code is the magma online thing and in both cases it spits out the same number: $-137$.
Here is the complete code.\newpage
\begin{verbatim}
sym := func< a,b | Binomial(b+a-1,a) >;

cohP1 := func< a | sym(a,2) - sym(-a-2,2) >;

cohP4 := func< a | sym(a,5) + sym(-a-5,5) >;

cohPP1 := function(v)
    if v[3] eq -1 then return 0;
    elif v[3] ge 0 then
        tmp1 := &+[cohP4(v[1]-h) : h in [0..v[3]]];
        return cohP1(v[2])*tmp1;
    elif -v[3] -2 ge 0 then
        tmp2 := &+[cohP4(v[1]+k+1) : k in [0..-v[3]-2]];
		return -cohP1(v[2])*tmp2;
    end if;
end function;

cohH := function(v)
    u := [v[1],v[2],v[1]+v[3]];
    w := [v[1]-3,v[2]-1,v[1]+v[3]-1];
    return cohPP1(u) - cohPP1(w);
end function;

hom := function(v,w)
    return cohH(w-v);
end function;

homF := func<v,x | cohP1(x-v[2]) >;

Fhom := func< x,v | cohP1(v[2]-x-1) >;

Gamma := func< v | cohH(v) - cohH(v+Vector([2,1,-3])) >;



a1 := 1;
A1 := 1;

a2 := 5;
A2 := Vector([4,1,-2]);

a3 := -10;
A3 := Vector([3,1,-2]);

a4 := -1;
A4 := Vector([5,1,-2]);

a5 := 0;
A5 := Vector([2,1,-1]);

a6 := 0;
A6 := Vector([1,1,0]);

a7 := 0;
A7 := Vector([2,0,-1]);

a8 := 0;
A8 := Vector([1,0,0]);

A := [Vector([0,0,0]),A2,A3,A4,A5,A6,A7,A8];
a := [a1,a2,a3,a4,a5,a6,a7,a8];


a5 := -(homF(A5,A1) + &+[a[i]*hom(A5,A[i]) : i in [2..4]]);
a := [a1,a2,a3,a4,a5,a6,a7,a8];
a6 := -(homF(A6,A1) + &+[a[i]*hom(A6,A[i]) : i in [2..5]]);
a := [a1,a2,a3,a4,a5,a6,a7,a8];
a7 := -(homF(A7,A1) + &+[a[i]*hom(A7,A[i]) : i in [2..6]]);
a := [a1,a2,a3,a4,a5,a6,a7,a8];
a8 := -(homF(A8,A1) + &+[a[i]*hom(A8,A[i]) : i in [2..7]]);
a := [a1,a2,a3,a4,a5,a6,a7,a8];

r1 := a1*(cohP1(A1) - cohP1(A1+1)) + &+[a[i]*Gamma(A[i]) : i in [2..8]];

print "Left mutating we get", r1;



B1 := 0;
b1 := 1;

B2 := Vector([1,0,0]);
b2 := 5;

B3 := Vector([0,0,0]);
b3 := -10;

B4 := Vector([2,0,0]);
b4 := -1;

B5 := Vector([0,0,0]);
b5 := 0;

B6 := Vector([1,0,-1]);
b6 := 0;

B7 := Vector([2,0,-2]);
b7 := 0;

B8 := Vector([0,1,0]);
b8 := 0;

B9 := Vector([1,1,-1]);
b9 := 0;

B10 := Vector([2,1,-2]);
b10 := 0;

B := [Vector([0,0,0]),B2,B3,B4,B5,B6,B7,B8,B9,B10];
b := [b1,b2,b3,b4,b5,b6,b7,b8,b9,b10];

b5 := -(Fhom(B1,B5) + &+[b[i]*hom(B[i],B5) : i in [2..10]]);
b := [b1,b2,b3,b4,b5,b6,b7,b8,b9,b10];
b6 := -(Fhom(B1,B6) + &+[b[i]*hom(B[i],B6) : i in [2..10]]);
b := [b1,b2,b3,b4,b5,b6,b7,b8,b9,b10];
b7 := -(Fhom(B1,B7) + &+[b[i]*hom(B[i],B7) : i in [2..10]]);
b := [b1,b2,b3,b4,b5,b6,b7,b8,b9,b10];
b8 := -(Fhom(B1,B8) + &+[b[i]*hom(B[i],B8) : i in [2..10]]);
b := [b1,b2,b3,b4,b5,b6,b7,b8,b9,b10];
b9 := -(Fhom(B1,B9) + &+[b[i]*hom(B[i],B9) : i in [2..10]]);
b := [b1,b2,b3,b4,b5,b6,b7,b8,b9,b10];
b10 := -(Fhom(B1,B10) + &+[b[i]*hom(B[i],B10) : i in [2..10]]);
b := [b1,b2,b3,b4,b5,b6,b7,b8,b9,b10];

r2 := b1*cohP1(B1) - b1*cohP1(B1+1) + &+[b[i]*Gamma(B[i]) : i in [2..10]];
print "Right mutating we get", r2;
\end{verbatim}








\newpage
\begin{flalign}
&& \xi\coloneqq \O_F(1) + 5\O(4,1)(-2e) -10 \O(3,1)(-2e) - \O(5,1)(-2e)
\end{flalign}

$\Hom(\O(2,1)(-e),\O_F(1))=1$

$\Hom(\O(2,1)(-e),\O(4,1)(-2e))= 20$

$\Hom(\O(2,1)(-e),\O(3,1)(-2e))=5$

$\Hom(\O(2,1)(-e),\O(5,1)(-2e))=55$

\begin{flalign}
&& \mu_1 \xi = \O_F(1) +4 \O(2,1)(-e) + 5 \O(4,1)(-2e) - 10\O(3,1)(-2e) - \O(5,1)(-2e)
\end{flalign}

$\Hom(\O(1,1),\O_F(1))=1$

$\Hom(\O(1,1),\O(2,1)(-e)=5$

$\Hom(\O(1,1),\O(4,1)(-2e))=50$

$\Hom(\O(1,1),\O(3,1)(-2e))= 15$ 

$\Hom(\O(1,1),\O(5,1)(-2e))=120$

\begin{flalign}
&& \mu_2\mu_1 \xi = \\ \notag &&
    \O_F(1) 
    - \O(2,1)(-e) 
    + 5\O(4,1)(-2e)
    -10 \O(3,1)(-2e)
    -\O(5,1)(-2e)
    -\O(1,1)
\end{flalign}

$\Hom(\O(2,0)(-e),\O_F(1))=2$

$\Hom(\O(2,0)(-e),\O(2,1)(-e))=2$

$\Hom(\O(2,0)(-e),\O(4,1)(-2e))=40$

$\Hom(\O(2,0)(-e),\O(3,1)(-2e))=40$

$\Hom(\O(2,0)(-e),\O(5,1)(-2e))=109$

$\Hom(\O(2,0)(-e),\O(1,1))=0$

\begin{flalign}
&& \mu_3\mu_3\mu_1 \xi = \\ \notag
&& \O_F(1) 
    - \O(2,1)(-e) 
    + 5\O(4,1)(-2e)
    -10 \O(3,1)(-2e)
    -\O(5,1)(-2e)
    -\O(1,1) \\ \notag &&
    +309 \O(2,0)(-e)
\end{flalign}

$\Hom(\O(1,0),\O_F(1))= 2$

$\Hom(\O(1,0),\O(2,1)(-e))= 10$

$\Hom(\O(1,0),\O(4,1)(-2e))=99$

$\Hom(\O(1,0),\O(3,1)(-2e))=30$

$\Hom(\O(1,0),\O(5,1)(-2e))=234$

$\Hom(\O(1,0),\O(1,1))=2$

$\Hom(\O(1,0),\O(2,0)(-e))=5$

\begin{flalign}
&& \mu_4\mu_3\mu_2\mu_1 \xi = \\ \notag
&& 
\O_F(1) 
    - \O(2,1)(-e) 
    + 5\O(4,1)(-2e)
    -10 \O(3,1)(-2e)
    -\O(5,1)(-2e)
    - \O(1,1) \\ \notag &&
    +309\O(2,0)(-e)
    -1496 \O(1,0)
\end{flalign}
\todo[inline,color=red]{STOP}
To proceed we project to $Y$ and then push into $\P^4 \times \P^1$ by applying $\gamma_*i_*i^!$ and in the K-group we have
\[ \Phi(\E) = \gamma_* i_* i^! (\E) = \gamma_* \E - \gamma_* \E \otimes \O(2,1)(-3e) \]
Since we want to check the Euler characteristic, we might as well push down to a point, ie compute
$H^*(\H,\E) - H^*(\H,\E \otimes \O(2,1)(-3e))$.
\begin{itemize}
\item $-1$
\item $0$
\item $104055$
\item $-939400$
\item $-294480$
\item $-3372$
\end{itemize}
which would seem negative.

\todo[inline,color=red]{END --- STOP READING}


\begin{align*}
\Phi(\O_F(1)) &= \gamma_* \O_F(1) - \gamma_* \O_F(2) = -\O_p \\
-\Phi\O(2,1)(-e) &= 
    -\O(2,1)
    -\O(1,1)
    +\O(-1,0)
    +\O(4,2) \\
5\Phi \O(4,1)(-2e) &=
    +5\O(4,1)
    +5\O(3,1)
    +5\O(2,1)
    -5\O(1,0)
    -5\O
    -5\O(6,2)
    -5\O(5,2)
    +5\O(3,1) \\
-10\O(3,1)(-2e) &=
    -10\O(3,1)
    -10\O(2,1)
    +10\O
    +10\O(5,2) \\
-\Phi(\O(5,1)) &=
\end{align*}


\begin{align*}
\gamma_* \O(x,y)(ze) = \\
\O(x,y)\otimes \rho_* \O_\rho(z) - \O(x-3,y-1)\otimes \rho_* \O_\rho(z-1) \\
\sum_{0 \leq h \leq z } \O(x-h,y)
-\sum_{0 \leq k \leq -z -2} \O(1+x+k,y)
-\sum_{0 \leq j \leq z-1} \O(x-3-j,y-1)
+\sum_{0 \leq l \leq -z-1} \O(x+l-2,y-1)
\end{align*}
We want 
\[ \Phi \mu_4 \mu_3 \mu_3 \mu_1 \O_F(1) = \Phi \big( \O_F(1) - \O(1,1) - \O(2,1)(-e) \big) \]

$\Phi(\O_F(1)) = \gamma_* \O_F(1) - \gamma_* \O_F(1) \otimes \O(2,1)(2e) $
so that
\begin{align}
\Phi(\O_F(1)) = \O_F(1) - \O_F(2) = -\O_p
\end{align}
where $p$ is a point of $W \times L$.

$ \Phi(\O(1,1)) = \gamma_* \O(1,1) - \gamma_* \O(3,2)(2e) $
so that
\begin{align}
-\Phi(\O(1,1)) = -\O(1,1) + \O(3,2) + \O(2,2) + \O(1,2) - \O(0,1) - \O(-1,1)
\end{align}


$\Phi(\O(2,1)(-e)) = \gamma_* \O(2,1)(-e) - \gamma_*\O(4,2)(e)$
so that
\begin{align}
-\Phi(\O(2,1)(-e)) = -\O + \O(4,2) + \O(3,2) - \O(1,1)
\end{align}

\bigskip
Collecting them all together we have
\begin{align*}
\Phi(\O_F(1)) &= \O_F(1) - \O_F(2) = -\O_p \\
-\Phi(\O(1,1)) &= -\O(1,1) + \O(3,2) + \O(2,2) + \O(1,2) - \O(0,1) - \O(-1,1) \\
-\Phi(\O(2,1)(-e)) &= -\O + \O(4,2) + \O(3,2) - \O(1,1)
\end{align*}

It would then seem that
\[ \Phi(\O_F(1)) = -\O_p  - 2\O(1,1) -\O(0,1) - \O(-1,1) - \O + 2 \O(3,2) + \O(2,2) + \O(1,2) + \O(4,2) \]
Let's compute the rank (Euler characteristic) of its cohomology.
\begin{align*}
-\O_p &= -1 \\
-2\O(1,1) &= -20 \\
-\O(0,1)  &= -2 \\
-\O(-1,1) &= 0 \\
-\O &= -1 \\
2\O(3,2) &= 210 \\
\O(2,2) &= 45 \\
\O(1,2) &= 30 \\
\O(4,2) &= 5
\end{align*}
which adds up to $266$.
I'm not sure how to interpret that sum in the K-group though, other than saying things like $\O(3,2) - \O(1,1)$ is the same as $\O_A(1,0)$ for $A$ a $(1,1)$ hypersurface etc.



\section{old}
\begin{align*}
    \O(e) &= \O_\rho(1) \\
    \O(x,y)(ze) &= \gamma^* \O(x,y)\otimes \alpha^* \O_\rho(x+z) \\
    \O(-\H) &= \O(-3,-1)(2e) = \rho^* \O(-3,-1)\otimes \O_\rho(-1) \\
    K_\H &= \O(-3,-1)(2e) \\
        &= \gamma^* \O(-3,-1)\otimes \alpha^*\O_\rho(-1) \\
        &= \gamma^* \O(-5,-2)(D) \\
        \O(-D) &= 
            \O(-2,-1)(3e) \\ &= \gamma^* \O(-2,-1)\otimes \alpha^*\O_\rho(1) \\
        K_D &= i^* \big( \gamma^* \O(-1,0) \otimes \alpha^* \O_\rho(-2) \big) \\
        i^!(-) &= \otimes K_D [4] \circ i^* \circ \otimes K_\H^{-1} [-5] \\
        &= i^* \big( (-) \otimes \gamma^* \O(2,1) \otimes \alpha^* \O_\rho(-1) \big)[-1]
\end{align*}




So,
\begin{align*}
%H^*(L,\O(y)) \otimes H^*(W, \O(x) \otimes \rho_* \O_\rho(z))
H^*\big( P\times \P^1, \rho^* \O(x,y) \otimes \O_\rho(z) \big) =
\big[ \Sym^y \C^2 \oplus \Sym^{-y-2} \C^2 [-1] \big]
\otimes \\
\left[
    \bigoplus_{0 \leq h \leq z} 
        \big( \Sym^{x-h} \C^5 \oplus \Sym^{-x+h-5} \C^5[-4] \big) 
    \oplus
    \bigoplus_{0 \leq k \leq -z-2}
        \big( \Sym^{1+x+k} \C^5[-1] \oplus \Sym^{-x-k-6}\C^5[-5] \big)
\right]
\end{align*}

\bigskip
In the K-group a mutation $L_E F$ becomes
\[ [L_E F] = [F] - \chi [E] \]
where $\chi$ is the Euler characteristic of $\Hom(E,F)$.


so we have (I'm taking $\chi$)
\begin{align*}
H^* \big( \H, \gamma^* \O(x,y) \otimes \alpha^* \O_\rho (z) \big) = \\
H^*\big( P \times L, \rho^*\O(x,y) \otimes \O_\rho (z) \big) - 
H^*\big( P\times L, \rho^* \O(x-3,y-1) \otimes \O_\rho (z-1) \big)
\end{align*}
Finally, let's have a formula for the bundles pushed to $\P^4 \times \P^1$ look like.
\begin{align*}
\gamma_*\big(  \gamma^*\O(x,y)\otimes \alpha^*\O_\rho(z) \big) = 
\gamma_* \O(x,y)((z-x)e) \\
\O(x,y)\otimes \rho_* \O_\rho(z) - \O(x-3,y-1)\otimes \rho_* \O_\rho(z-1) \\
\sum_{0 \leq h \leq z } \O(x-h,y)
-\sum_{0 \leq k \leq -z -2} \O(1+x+k,y)
-\sum_{0 \leq j \leq z-1} \O(x-3-j,y-1)
+\sum_{0 \leq l \leq -z-1} \O(x+l-2,y-1)
\end{align*}

It might be useful to recall
\begin{align*}
\Sym^a \C^2 &= a+1 \\
\Sym^2 \C^5 &= 15 \\
\Sym^3 \C^5 &= 35 \\
\Sym^4 \C^5 &= 70 \\
\Sym^5 \C^5 &= 126 \\
\Sym^6 \C^5 &= 210 \\
\Sym^7 \C^5 &= 330
\end{align*}
But let's start now.





\smallskip
Let's write compactly some useful cohomology groups.
\[ H^*(P^4, \O(x)) = \Sym^x \C^5 \oplus \Sym^{-x-5} \C^5[-4]\]

\[ H^*(\P^1,\O(y)) = \Sym^y \C^2 \oplus \Sym^{-y-2} \C^2 [-1]\]

\[ H^*(\P^4\times \P^1, \O(x,y) ) = H^*(\P^4,\O(x)) \otimes H^*(\P^1, \O(y)) \]
for any $x,y \in \Z$.

